Gaussian Billboards: Expressive 2D Gaussian Splatting with Textures

Gaussian Splatting has recently emerged as the go-to representation for reconstructing and rendering 3D scenes. The transition from 3D to 2D Gaussian primitives has further improved multi-view consistency and surface reconstruction accuracy. In this work we highlight the similarity between 2D Gaussian Splatting (2DGS) and billboards from traditional computer graphics. Both use flat semi-transparent 2D geometry that is positioned, oriented and scaled in 3D space. However 2DGS uses a solid color per splat and an opacity modulated by a Gaussian distribution, where billboards are more expressive, modulating the color with a uv-parameterized texture. We propose to unify these concepts by presenting Gaussian Billboards, a modification of 2DGS to add spatially-varying color achieved using per-splat texture interpolation. The result is a mixture of the two representations, which benefits from both the robust scene optimization power of 2DGS and the expressiveness of texture mapping. We show that our method can improve the sharpness and quality of the scene representation in a wide range of qualitative and quantitative evaluations compared to the original 2DGS implementation.

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{figures/teaser/Teaser.pdf}
    \caption{We propose a drop-in enhancement for 2D Gaussian Splatting that (a) replaces the per-primitive solid color with a small per-primitive texture. This allows the 2DGS to represent more details (b) when the number of primitives is fixed to, \eg, 100000. Even with the standard densification strategy and identical hyperparameters, it improves the quality of 3D scene reconstruction (c), shown on a test view.}
    \label{fig:teaser}
\end{figure*}

Neural scene representations have become a standard solution to represent arbitrary 3D scenes from a collection of 2D images, allowing for novel view synthesis, relighting, animation playback or animation retargeting, just to name a few applications.
Recently, 3D Gaussian Splatting (3DGS)~\cite{Kerbl2023-cv} has established itself as the method of choice, outperforming previous representations like NeRF~\cite{Mildenhall2020-mp} or Mixture of Volumetric Primitives~\cite{Lombardi2021-ah}.
3DGS's core idea is to represent the scene explicitly as a collection of volumetric primitives, positioned and oriented in 3D, and then rasterized and rendered as 2D splats on the screen. To make this representation differentiable, the opacity of this volume is modeled via a 3D Gaussian distribution.
%This avoids the edge discontinuities that other explicit mesh optimization techniques struggle with~\cite{Liu2019-ap,Laine2020-sx}.

Since the introduction of 3DGS, many improvements to its rendering and representation quality have been presented. In particular, 2D Gaussian Splatting (2DGS)~\cite{Huang2024-2dgs} replaces the volumetric primitives with oriented 2D primitives (disks).
Still, representing highly detailed textured areas with potentially low geometric details, \ie an image on a wall, remains challenging.

Looking back at traditional Computer Graphics, billboards have been a common staple for rendering complicated, semi-transparent features like leaves, grass, or particle effects in general.
We want to highlight here the similarities between 2DGS and billboards: in 2DGS, primitives are oriented 2D disks with a position, orientation and size in 3D, a constant color and opacity defined by a Gaussian distribution. Billboards are typically 2D squares with a position, orientation and size in 3D and a spatially-varying color and opacity using texture mapping.

To combine the best of both representations, we present \textit{Gaussian Billboards}, an improvement over 2DGS in which the color of the splat is spatially modulated using a small per-primitive texture, see \cref{fig:teaser}a.
We show that replacing the per-primitive solid color with a per-primitive texture improves the reconstruction capability when a fixed number of primitives is employed (see \cref{fig:teaser}b), and also when the number of primitives is changed over the course of the optimization with densification and pruning strategies (see \cref{fig:teaser}c).
In short, our contributions are:
\begin{enumerate}
    \item A modification of 2DGS with a spatially-varying color defined by a per-primitive texture,
    \item A detailed ablation of the introduced hyperparameters,
    \item An evaluation of 2D and 3D scene representations showing the improved capabilities of Gaussian Billboards in representing texture details.
\end{enumerate}
%
It is worth mentioning that, while these contributions are novel, concurrent work by Rong~\etal~\cite{Rong2024-yq} named \textit{GStex} also explores similar ideas to enhance 2DGS with spatially varying textures.

